BatchGNN: Efficient CPU-Based Distributed GNN Training on Very Large Graphs

We present BatchGNN, a distributed CPU system that showcases techniques that can be used to efficiently train GNNs on terabyte-sized graphs. It reduces communication overhead with macrobatching in which multiple minibatches' subgraph sampling and feature fetching are batched into one communication relay to reduce redundant feature fetches when input features are static. BatchGNN provides integrated graph partitioning and native GNN layer implementations to improve runtime, and it can cache aggregated input features to further reduce sampling overhead. BatchGNN achieves an average $3\times$ speedup over DistDGL on three GNN models trained on OGBN graphs, outperforms the runtimes reported by distributed GPU systems $P^3$ and DistDGLv2, and scales to a terabyte-sized graph.

==> related_work.tex <==
\subsection{Distributed GNN Systems}

In order to scale out GNN computation to large models and graphs, distributed
GNN systems (including single-machine multi-device systems) divide the data
and/or the computation among multiple devices in various ways.
CPU-focused systems include Graph-Learn~\cite{AliGraph},
DistGNN~\cite{DistGNN}, DeepGalois~\cite{deepgalois}, DistDGL~\cite{distdgl},
Euler~\cite{eulergnn}, and ByteGNN~\cite{bytegnn}
(note DistDGL and Euler can run on GPUs as well).
GPU-focused systems include DistDGLv2~\cite{distdglv2}, PaGraph~\cite{pagraph},
NeuGraph~\cite{ma2019neugraph}, Roc~\cite{rocgnn}, CAGNET~\cite{CAGNET},
SALIENT~\cite{SALIENT}, and $P^3$~\cite{p3}

These systems have different methods of distributing the computation and data
associated with GNN training.  For instance, SALIENT~\cite{SALIENT} does not do
any partitioning of the graph and assumes that it all fits into memory, and
computation is distributed among devices. This
does not work for large graphs.  Most systems do graph partitioning 
to avoid this problem, and the partitioning policy used determines
the amount of communication among devices that needs to occur. 
For example, systems like \systemname{} and DistDGL~\cite{distdgl} partition the
graph topology and assign entire vertex features to a single machines, and the
topology and features are communicated to other machines during subgraph
sampling. $P^3$~\cite{p3} distributes the topology and its features such that a
single machine may not have a vertex's entire feature, and to do computation,
sampled subgraphs are communicated to all machines so that each machine can use
its partition of the features to do partial computation of results.
ByteGNN~\cite{bytegnn} partitions the graph based
on a breadth-first search on training/validation/test vertices
and uses scheduler-managed threads to sample many subgraphs in parallel.
CAGNET~\cite{CAGNET} distributes and communicates data such that the blocks of the
adjacency matrix (i.e., the graph) and feature matrix are
communicated in a manner similar to doing distributed matrix multiply. 
Finally, systems like Graph-Scope~\cite{graphscope} (which includes
Graph-Learn~\cite{AliGraph}) can access a distributed in-memory Vineyard store that
contains the graph and any data needed for compute.

\subsection{GNN Sampling Schemes}

Many sampling schemes have been proposed in order to reduce the computational
and memory costs of full-neighbor GNN training.

GraphSAGE~\cite{graphsage} samples a fixed number of neighbors for
every node in the previous sampling layer and constructs an individual subgraph
for each layer using the sampled edges/neighbors; this is what \systemname{}
uses.  GraphSAINT~\cite{GraphSAINT} samples a set of nodes (random node,
random edge, or random walk), and the subgraph induced from
those nodes is the subgraph used for \emph{all} GNN layers (sampling occurs over
the subgraph as necessary).  FastGCN~\cite{fastgcn} does independent layer
sampling where each layer independently samples a fixed set of nodes based on
some probability distribution (e.g., degree-based) and uses the induced subgraph
of the sampled nodes at each layer. Sampling a fixed amount per layer avoids
exponential growth of neighbors that can occur in GraphSAGE.  Layer-dependent
importance sampling (LADIES)~\cite{ladies_sampling} improves FastGCN by sampling
nodes that are neighbors of the previous sampled layer which addresses an issue
in FastGCN in which it could sample disconnected nodes.
Influence-based minibatching~\cite{sampleibmb} creates static minibatches 
that sample only the most influential vertices of a seed vertex via personalized
page rank to improve accuracy and runtime.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Approximate Distributed GNN Training}

Because feature communication during distributed training can be a
bottleneck, researchers have proposed methods to reduce the overhead via
\emph{approximate} training. These methods change the semantics of training and
can be applied orthogonally to existing systems.  DistGNN~\cite{DistGNN} allows
stale features on vertices during training, so vertex features do not
need to be continuously updated.  BNS-GCN~\cite{bns-gcn}
only communicates a sampled subset of the boundary vertices that require updated
features.  GNNAutoScale~\cite{gnnautoscale} uses features from previous 
epochs to approximate features beyond a vertex's 1-hop neighborhood.

\systemname{}'s input feature aggregation cache can be considered a form of
approximate training in the sampling setting since it replaces sampled
aggregation with full-neighborhood cached aggregation to avoid the
costs associated with sampling for the first computational layer. It is not
approximate training, however, when used in a setting where all neighbors
are aggregated over since the cached aggregation would be accurate in that setting.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

